How Lightning's Routing Diminishes its Anonymity

The system shows the error of "Bad character(s) in field Abstract" for no reason. Please refer to manuscript for the full abstract

==> ACM%20Conference%20Proceedings%20Primary%20Article%20Template%20(2)-2/attack-exampleShortest.tex <==
\begin{tikzpicture}
\draw[fill=gray!10] (0,0) rectangle (7.5,4);

%sets 
\draw[blue,fill=white,line width=0.0mm] (5.8,1.5) ellipse (1.3cm and 1.3cm);
\node[text width=2.5cm] at (6,3.1) {\small \baselineskip=7pt Receiver Anonymity Set \par}; 
\draw[blue,fill=white,line width=0.0mm] (2.7,2.1) ellipse (0.9cm and 0.95cm);
\node[text width=2.2cm] at (2.5,3.4) {\small \baselineskip=7pt Sender Anonymity Set \par}; 

%nodes 
\node[mynode,fill=blue!20] at (1.5,  1.5)(a){}; 
\node[mynode,fill=blue!20] at (3,  1.5)(pre){};
\node[mynode,fill=red!60] at (4,  1.5)(A){A};
\node[mynode,fill=blue!20] at (5,  1.5)(nxt){};
\node[mynode,fill=blue!20] at (6,  0.5)(dstA){};
\node[mynode,fill=blue!20] at (6,  2.5)(dstB){};
\node[mynode,fill=blue!20] at (4.1,  0.5)(below){};
\node[mynode,fill=blue!20] at (2.25,  2.5)(upA){};
\node[mynode,fill=blue!20] at (3.1,  2.5)(upB){};
\node[mynode,fill=blue!20] at (3.9,  2.5)(upC){};

%edges 
\draw[black,line width=0.5mm] (a) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (A);
\draw[black,line width=0.5mm] (A) -- (nxt);
\draw[black,line width=0.5mm] (a) -- (upA);
\draw[black,line width=0.5mm] (a) -- (below);
\draw[black,line width=0.5mm] (upA) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (upB);
\draw[black,line width=0.5mm] (upB) -- (upC);
\draw[black,line width=0.5mm] (upC) -- (A);
\draw[black,line width=0.5mm] (A)  -- (below);
\draw[black,line width=0.5mm] (below) -- (nxt);
\draw[black,line width=0.5mm] (nxt) -- (dstA);
\draw[black,line width=0.5mm] (nxt) -- (dstB);
\draw[black,line width=0.5mm] (dstA) -- (dstB);  

%att observation 
\draw[red,line width=0.5mm, ->] (3.2,1.4) -- (3.8,1.4); 
\draw[red,line width=0.5mm, ->] (4.2,1.4) -- (4.8,1.4); 



%legend 
\draw[black,line width=0.5mm,label=right] (0.1,0.7) -- (0.5,0.7) node[right]{\small Channel};  
\draw[red,line width=0.5mm, ->,label=right] (0.1,0.3) -- (0.5,0.3) node[right]{\small \textcolor{black}{Payment Observation}};  
\end{tikzpicture}

==> ACM%20Conference%20Proceedings%20Primary%20Article%20Template%20(2)-2/attack-timeout.tex <==
\begin{tikzpicture}
\draw[fill=gray!10] (0,0) rectangle (7.5,4);

%sets 
\draw[blue,fill=white,line width=0.0mm] (6,1.5) ellipse (0.6cm and 1.3cm);
\node[text width=2.5cm] at (6,3.1) {\small \baselineskip=7pt Receiver Anonymity Set \par}; 
\draw[blue,fill=white,line width=0.0mm] (2.7,2.1) ellipse (0.9cm and 0.95cm);
\node[text width=2.2cm] at (2.5,3.4) {\small \baselineskip=7pt Sender Anonymity Set \par}; 

%nodes 
\node[mynode,fill=blue!20] at (1.5,  1.5)(a){3}; 
\node[mynode,fill=blue!20] at (3,  1.5)(pre){2};
\node[mynode,fill=red!60] at (4,  1.5)(A){2};
\node[mynode,fill=blue!20] at (5,  1.5)(nxt){4};
\node[mynode,fill=blue!20] at (6,  0.5)(dstA){3};
\node[mynode,fill=blue!20] at (6,  2.5)(dstB){3};
\node[mynode,fill=blue!20] at (4.1,  0.5)(below){5};
\node[mynode,fill=blue!20] at (2.25,  2.5)(upA){3};
\node[mynode,fill=blue!20] at (3.1,  2.5)(upB){1};
\node[mynode,fill=blue!20] at (3.9,  2.5)(upC){3};

%edges 
\draw[black,line width=0.5mm] (a) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (A);
\draw[black,line width=0.5mm] (A) -- (nxt);
\draw[black,line width=0.5mm] (a) -- (upA);
\draw[black,line width=0.5mm] (a) -- (below);
\draw[black,line width=0.5mm] (upA) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (upB);
\draw[black,line width=0.5mm] (upB) -- (upC);
\draw[black,line width=0.5mm] (upC) -- (A);
\draw[black,line width=0.5mm] (A)  -- (below);
\draw[black,line width=0.5mm] (below) -- (nxt);
\draw[black,line width=0.5mm] (nxt) -- (dstA);
\draw[black,line width=0.5mm] (nxt) -- (dstB);
\draw[black,line width=0.5mm] (dstA) -- (dstB);  

%att observation 
\draw[red,line width=0.5mm, ->] (3.2,1.4) -- (3.8,1.4) node[midway,below]{9}; 
\draw[red,line width=0.5mm, ->] (4.2,1.4) -- (4.8,1.4) node[midway,below]{7};; 
%\node at (3.5,1.3)(lab){\small \textbf{\textcolor{red}{9}}}; 




%legend 
\draw[black,line width=0.5mm,label=right] (0.1,0.7) -- (0.5,0.7) node[right]{\small Channel};  
\draw[red,line width=0.5mm, ->,label=right] (0.1,0.3) -- (0.5,0.3) node[right]{\small \textcolor{black}{Payment Observation}};  
\end{tikzpicture}

==> ACM%20Conference%20Proceedings%20Primary%20Article%20Template%20(2)-2/macros.tex <==
%%Network
\newcommand{\nodes}{N}
\newcommand{\capacity}{c}
\newcommand{\bal}{bal}
\newcommand{\source}{S}
\newcommand{\receiver}{R}
\newcommand{\base}{b}
\newcommand{\feerate}{f}
\newcommand{\delay}{d}

%%Attacker
\newcommand{\att}{\mathbf{A}}
\newcommand{\anonymityset}{C}
\newcommand{\timeout}{t}




%%notes
\newcommand{\stef}[1]{{\color{orange}Stef: #1}}
\newcommand{\stefSerious}[1]{{\color{red}Stef: #1}}
\newcommand{\satw}[1]{{\color{blue} Satw: #1}}

==> attack-exampleShortest.tex <==
\begin{tikzpicture}
\draw[fill=gray!10] (0,0) rectangle (7.5,4);

%sets 
\draw[blue,fill=white,line width=0.0mm] (5.8,1.5) ellipse (1.3cm and 1.3cm);
\node[text width=2.5cm] at (6,3.1) {\small \baselineskip=7pt Receiver Anonymity Set \par}; 
\draw[blue,fill=white,line width=0.0mm] (2.7,2.1) ellipse (0.9cm and 0.95cm);
\node[text width=2.2cm] at (2.5,3.4) {\small \baselineskip=7pt Sender Anonymity Set \par}; 

%nodes 
\node[mynode,fill=blue!20] at (1.5,  1.5)(a){}; 
\node[mynode,fill=blue!20] at (3,  1.5)(pre){};
\node[mynode,fill=red!60] at (4,  1.5)(A){A};
\node[mynode,fill=blue!20] at (5,  1.5)(nxt){};
\node[mynode,fill=blue!20] at (6,  0.5)(dstA){};
\node[mynode,fill=blue!20] at (6,  2.5)(dstB){};
\node[mynode,fill=blue!20] at (4.1,  0.5)(below){};
\node[mynode,fill=blue!20] at (2.25,  2.5)(upA){};
\node[mynode,fill=blue!20] at (3.1,  2.5)(upB){};
\node[mynode,fill=blue!20] at (3.9,  2.5)(upC){};

%edges 
\draw[black,line width=0.5mm] (a) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (A);
\draw[black,line width=0.5mm] (A) -- (nxt);
\draw[black,line width=0.5mm] (a) -- (upA);
\draw[black,line width=0.5mm] (a) -- (below);
\draw[black,line width=0.5mm] (upA) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (upB);
\draw[black,line width=0.5mm] (upB) -- (upC);
\draw[black,line width=0.5mm] (upC) -- (A);
\draw[black,line width=0.5mm] (A)  -- (below);
\draw[black,line width=0.5mm] (below) -- (nxt);
\draw[black,line width=0.5mm] (nxt) -- (dstA);
\draw[black,line width=0.5mm] (nxt) -- (dstB);
\draw[black,line width=0.5mm] (dstA) -- (dstB);  

%att observation 
\draw[red,line width=0.5mm, ->] (3.2,1.4) -- (3.8,1.4); 
\draw[red,line width=0.5mm, ->] (4.2,1.4) -- (4.8,1.4); 



%legend 
\draw[black,line width=0.5mm,label=right] (0.1,0.7) -- (0.5,0.7) node[right]{\small Channel};  
\draw[red,line width=0.5mm, ->,label=right] (0.1,0.3) -- (0.5,0.3) node[right]{\small \textcolor{black}{Payment Observation}};  
\end{tikzpicture}

==> attack-timeout.tex <==
\begin{tikzpicture}
\draw[fill=gray!10] (0,0) rectangle (7.5,4);

%sets 
\draw[blue,fill=white,line width=0.0mm] (6,1.5) ellipse (0.6cm and 1.3cm);
\node[text width=2.5cm] at (6,3.1) {\small \baselineskip=7pt Receiver Anonymity Set \par}; 
\draw[blue,fill=white,line width=0.0mm] (2.7,2.1) ellipse (0.9cm and 0.95cm);
\node[text width=2.2cm] at (2.5,3.4) {\small \baselineskip=7pt Sender Anonymity Set \par}; 

%nodes 
\node[mynode,fill=blue!20] at (1.5,  1.5)(a){3}; 
\node[mynode,fill=blue!20] at (3,  1.5)(pre){2};
\node[mynode,fill=red!60] at (4,  1.5)(A){2};
\node[mynode,fill=blue!20] at (5,  1.5)(nxt){4};
\node[mynode,fill=blue!20] at (6,  0.5)(dstA){3};
\node[mynode,fill=blue!20] at (6,  2.5)(dstB){3};
\node[mynode,fill=blue!20] at (4.1,  0.5)(below){5};
\node[mynode,fill=blue!20] at (2.25,  2.5)(upA){3};
\node[mynode,fill=blue!20] at (3.1,  2.5)(upB){1};
\node[mynode,fill=blue!20] at (3.9,  2.5)(upC){3};

%edges 
\draw[black,line width=0.5mm] (a) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (A);
\draw[black,line width=0.5mm] (A) -- (nxt);
\draw[black,line width=0.5mm] (a) -- (upA);
\draw[black,line width=0.5mm] (a) -- (below);
\draw[black,line width=0.5mm] (upA) -- (pre);
\draw[black,line width=0.5mm] (pre) -- (upB);
\draw[black,line width=0.5mm] (upB) -- (upC);
\draw[black,line width=0.5mm] (upC) -- (A);
\draw[black,line width=0.5mm] (A)  -- (below);
\draw[black,line width=0.5mm] (below) -- (nxt);
\draw[black,line width=0.5mm] (nxt) -- (dstA);
\draw[black,line width=0.5mm] (nxt) -- (dstB);
\draw[black,line width=0.5mm] (dstA) -- (dstB);  

%att observation 
\draw[red,line width=0.5mm, ->] (3.2,1.4) -- (3.8,1.4) node[midway,below]{9}; 
\draw[red,line width=0.5mm, ->] (4.2,1.4) -- (4.8,1.4) node[midway,below]{7};; 
%\node at (3.5,1.3)(lab){\small \textbf{\textcolor{red}{9}}}; 




%legend 
\draw[black,line width=0.5mm,label=right] (0.1,0.7) -- (0.5,0.7) node[right]{\small Channel};  
\draw[red,line width=0.5mm, ->,label=right] (0.1,0.3) -- (0.5,0.3) node[right]{\small \textcolor{black}{Payment Observation}};  
\end{tikzpicture}
